A numerical comparison of the method of moments for the population balance equation

We investigate the application of the method of moments approach for the one-dimensional population balance equation. We consider different types of moment closures, namely polynomial (P_N) closures, maximum entropy (M_N) closures and the quadrature method of moments QMOM_N. Realizability issues and implementation details are discussed. The numerical examples range from spatially homogeneous cases to a population balance equation coupled with fluid dynamic equations for a lid-driven cavity test case. A detailed numerical discussion of accuracy, order of the moment method and computational time is given.

==> cbtest.tex <==
\def\mycolormap{                rgb(0pt)=(0.2081,0.1663,0.5292);
                rgb(1pt)=(0.211624,0.189781,0.577676);
                rgb(2pt)=(0.212252,0.213771,0.626971);
                rgb(3pt)=(0.2081,0.2386,0.677086);
                rgb(4pt)=(0.195905,0.264457,0.7279);
                rgb(5pt)=(0.170729,0.291938,0.779248);
                rgb(6pt)=(0.125271,0.324243,0.830271);
                rgb(7pt)=(0.0591333,0.359833,0.868333);
                rgb(8pt)=(0.0116952,0.38751,0.881957);
                rgb(9pt)=(0.00595714,0.408614,0.882843);
                rgb(10pt)=(0.0165143,0.4266,0.878633);
                rgb(11pt)=(0.0328524,0.443043,0.871957);
                rgb(12pt)=(0.0498143,0.458571,0.864057);
                rgb(13pt)=(0.0629333,0.47369,0.855438);
                rgb(14pt)=(0.0722667,0.488667,0.8467);
                rgb(15pt)=(0.0779429,0.503986,0.838371);
                rgb(16pt)=(0.0793476,0.520024,0.831181);
                rgb(17pt)=(0.0749429,0.537543,0.826271);
                rgb(18pt)=(0.0640571,0.556986,0.823957);
                rgb(19pt)=(0.0487714,0.577224,0.822829);
                rgb(20pt)=(0.0343429,0.596581,0.819852);
                rgb(21pt)=(0.0265,0.6137,0.8135);
                rgb(22pt)=(0.0238905,0.628662,0.803762);
                rgb(23pt)=(0.0230905,0.641786,0.791267);
                rgb(24pt)=(0.0227714,0.653486,0.776757);
                rgb(25pt)=(0.0266619,0.664195,0.760719);
                rgb(26pt)=(0.0383714,0.674271,0.743552);
                rgb(27pt)=(0.0589714,0.683757,0.725386);
                rgb(28pt)=(0.0843,0.692833,0.706167);
                rgb(29pt)=(0.113295,0.7015,0.685857);
                rgb(30pt)=(0.145271,0.709757,0.664629);
                rgb(31pt)=(0.180133,0.717657,0.642433);
                rgb(32pt)=(0.217829,0.725043,0.619262);
                rgb(33pt)=(0.258643,0.731714,0.595429);
                rgb(34pt)=(0.302171,0.737605,0.571186);
                rgb(35pt)=(0.348167,0.742433,0.547267);
                rgb(36pt)=(0.395257,0.7459,0.524443);
                rgb(37pt)=(0.44201,0.748081,0.503314);
                rgb(38pt)=(0.487124,0.749062,0.483976);
                rgb(39pt)=(0.530029,0.749114,0.466114);
                rgb(40pt)=(0.570857,0.748519,0.44939);
                rgb(41pt)=(0.609852,0.747314,0.433686);
                rgb(42pt)=(0.6473,0.7456,0.4188);
                rgb(43pt)=(0.683419,0.743476,0.404433);
                rgb(44pt)=(0.71841,0.741133,0.390476);
                rgb(45pt)=(0.752486,0.7384,0.376814);
                rgb(46pt)=(0.785843,0.735567,0.363271);
                rgb(47pt)=(0.818505,0.732733,0.34979);
                rgb(48pt)=(0.850657,0.7299,0.336029);
                rgb(49pt)=(0.882433,0.727433,0.3217);
                rgb(50pt)=(0.913933,0.725786,0.306276);
                rgb(51pt)=(0.944957,0.726114,0.288643);
                rgb(52pt)=(0.973895,0.731395,0.266648);
                rgb(53pt)=(0.993771,0.745457,0.240348);
                rgb(54pt)=(0.999043,0.765314,0.216414);
                rgb(55pt)=(0.995533,0.786057,0.196652);
                rgb(56pt)=(0.988,0.8066,0.179367);
                rgb(57pt)=(0.978857,0.827143,0.163314);
                rgb(58pt)=(0.9697,0.848138,0.147452);
                rgb(59pt)=(0.962586,0.870514,0.1309);
                rgb(60pt)=(0.958871,0.8949,0.113243);
                rgb(61pt)=(0.959824,0.921833,0.0948381);
                rgb(62pt)=(0.9661,0.951443,0.0755333);
                rgb(63pt)=(0.9763,0.9831,0.0538)}
